Detailed abundances in stars belonging to ultra-faint dwarf spheroidal galaxies

We report preliminary results concerning the detailed chemical composition of metal poor stars belonging to close ultra-faint dwarf galaxies (hereafter UfDSphs). The abundances have been determined thanks to spectra obtained with X-Shooter, a high efficiency spectrograph installed on one of the ESO VLT units. The sample of ultra-faint dwarf spheroidal stars have abundance ratios slightly lower to what is measured in field halo star of the same metallicity.We did not find extreme abundances in our Hercules stars as the one found by Koch for his 2 Hercules stars. The synthesis of the neutron capture elements Ba and Sr seems to originate from the same nucleosynthetic process in operation during the early stages of the galactic evolution.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

